Model-free Test Time Adaptation for Out-Of-Distribution Detection

Out-of-distribution (OOD) detection is essential for the reliability of ML models. Most existing methods for OOD detection learn a fixed decision criterion from a given in-distribution dataset and apply it universally to decide if a data point is OOD. Recent work~\cite{fang2022is} shows that given only in-distribution data, it is impossible to reliably detect OOD data without extra assumptions. Motivated by the theoretical result and recent exploration of test-time adaptation methods, we propose a Non-Parametric Test Time \textbf{Ada}ptation framework for \textbf{O}ut-Of-\textbf{D}istribution \textbf{D}etection (\abbr). Unlike conventional methods, \abbr utilizes online test samples for model adaptation during testing, enhancing adaptability to changing data distributions. The framework incorporates detected OOD instances into decision-making, reducing false positive rates, particularly when ID and OOD distributions overlap significantly. We demonstrate the effectiveness of \abbr through comprehensive experiments on multiple OOD detection benchmarks, extensive empirical studies show that \abbr significantly improves the performance of OOD detection over state-of-the-art methods. Specifically, \abbr reduces the false positive rate (FPR95) by $23.23\%$ on the CIFAR-10 benchmarks and $38\%$ on the ImageNet-1k benchmarks compared to the advanced methods. Lastly, we theoretically verify the effectiveness of \abbr.

==> sections/03_problem.tex <==




==> sections/04_method.tex <==

\textbf{Notation.} Given an input space $\mathcal{X}$, representation space $\mathcal{Z}$, and label space $\mathcal{Y}=\{1,2,...,c\}$, we have an ID dataset ${D}_{in}=\{(x_i,y_i)\}_{i=1}^N$ that is drawn from distribution $\mathcal{D}^{in}$. We have an OOD distribution $\mathcal{D}^{out}$ that is different from $\mathcal{D}^{in}$. We also have a feature encoder $h_\theta:\mathcal{X}\rightarrow \mathcal{Z}$ and classifier $f:\mathcal{Z}\rightarrow \mathbb{R}^c$, where $h_\theta,f$ are often parameterized by deep neural networks.

\textbf{Test-time Out-of-distribution (OOD) detection.} Given data $D_{in}$ sampled from ID $\mathcal{D}^{in}$, we train a neural network $h_\theta\circ f$. Our target is to construct a score function $S(x)$, which hopefully will assign higher scores for ID samples and lower scores for OOD samples. Formally, given a threshold $\lambda$ and input $x$, the decision that $x$ is from $\mathcal{D}^{in}$ is made by $\mathbf{I}\{S(x)\geq \lambda\}$, otherwise, $x$ is classified as an OOD sample. In this paper, like previous studies on OOD detection (e.g. ~\cite{yang2021generalized}), we assume that the labels of samples from $\mathcal{D}^{out}$ do not overlap with $\mathcal{D}^{in}$, which is often referred to as label shift. Unlike existing studies~\cite{yang2021generalized}, during inference, we propose not only to detect the OOD instances but also to utilize these samples to further improve the detection capability of our detectors.

\textbf{Difference between our method and existing OOD detectors.} The latter mainly includes (1) classification-based methods that derive OOD scores based on the classifier trained on ID data~\cite{hendrycks2016baseline}. Such as using the  maximum softmax probability~\cite{hendrycks2016baseline}, and energy~\cite{liu2020energy} as the OOD score. (2) Density-based methods model the ID with some probabilistic model and data samples lie in low-density regions are classified as OOD~\cite{zong2018deep,xiao2020likelihood}. and (3) Distance-based methods are based on an assumption that OOD samples should be relatively far away from the representation of ID classes~\cite{lee2018simple,wang2022vim}. Different from them, to our best knowledge, the proposed \abbr first seeks to utilize the online target data. In addition, there are some out-of-distribution detection methods that utilize auxiliary OOD data. This line of work regularizes the model during training~\cite{katz2022training}, which is different to our fully test-time adaptation setting, where we can exploit the benefit from the online test instances and attains much better performance. Due to the space limit, more related works are left in the appendix~\ref{sec:app_related}.


% \textbf{Motivation of test-time adaptation.} Recently, several impossibility theorems for the learnability of OOD detection under some scenarios are conducted~\cite{fang2022is}. These  frustrating theorems show that OOD detection can only learnable when the following strong assumptions hold.

% \begin{assump}
% \textit{(Linear Condition)} Given any mixed distribution $D=(1-\alpha)D_{in}+\alpha D_{out}$, where $D_{in}~\sim\mathcal{D}^{in}$ and $D_{out}~\sim\mathcal{D}^{out}$. A hypothesis space is a subset of functions that map the ID samples to the correct classes and OOD samples to the $c+1$-th class, i.e., $\mathcal{G}\subset\{g:\mathcal{X}\rightarrow \mathcal{Y}\cup\{c+1\}\}$. 
% \begin{gather}
% \inf_{g\in\mathcal{G}}R^\alpha_D(g)=(1-\alpha)\inf_{g\in\mathcal{G}}R^{in}_D(g)+\alpha\inf_{g\in\mathcal{G}}R^{out}_D(g),\notag
% \end{gather}
% where $R^{in}_D(g):=\mathbb{E}_{(x,y)\in D_{in}} \ell(g(x),y)$, $R^{out}_D(g):=\mathbb{E}_{(x,y)\in D_{out}} \ell(g(x),c+1)$, and $\ell$ is a loss function satisfying $\ell(y_1,y_2)=0$ if and only if $y_1=y_2$.
% \label{assump1}
% \end{assump}
% \begin{assump}
% \textit{(Compatibility)} For any small value $\nu$, there exists a hypothesis function $g_\nu\in\mathcal{G}$ such that
% \begin{gather}
% g_\nu\in\{g'\in\mathcal{G}:R^{out}_D(g')\leq\inf_{g\in\mathcal{G}}R^{out}_D(g)+\nu\} \cap \notag \\
% \{g'\in\mathcal{G}:R^{in}_D(g')\leq\inf_{g\in\mathcal{G}}R^{in}_D(g)+\nu\}, \notag
% \end{gather}
% where this assumption is a general version of Assumption~\ref{assump1}(Lemma 2 of~\cite{fang2022is}).
% \label{assump2}
% \end{assump}

% Only when Assumption~\ref{assump1} and Assumption~\ref{assump2} are satisfied, the OOD detection problem is PAC-learnable. However, these assumptions are unrealistic because we do not know (1) Whether there exists an optimal hypothesis $g_v$ that performs well on both $D_{in}$ and $D_{out}$? (2) If we can find the optimal hypothesis given only ID dataset? If the answer to the first question is ``no'', then almost all algorithms cannot solve the OOD detection problem successfully. In this section, we focus on the second problem and show that, even if $g_\nu$ exists, it is almost impossible to find it without OOD samples.
\vspace{-0.15cm}
\subsection{Motivation of test-time adaptation.} 
\vspace{-0.15cm}


As discussed in the introduction, without $\mathcal{D}^{out}$, a fixed decision threshold (i.e. $x = 1.96$) independent of test samples may not work well, particularly when the ID and OOD distributions overlap significantly. On the other hand, using the test samples labeled as OOD by our detection algorithm, we can obtain an estimation of $\mathcal{D}^{out}$ and reduce the decision threshold to $x=1.35$. It will result in the correct classification of $91\%$ ID samples and $90\%$ OOD samples, a significant improvement in OOD detection ($40\%$) at a small sacrifice of classification accuracy for ID samples ($4\%$).
\begin{wrapfigure}{r}{0.245\textwidth}
  \begin{center}
    \vspace{-0.2in}  
    \includegraphics[width=0.245\textwidth]{imgs/motivation_oodsample.pdf}
    \vspace{-0.2in} 
    \caption{FPR considering different available OOD samples.}
        \label{fig:motivation_ood}
    \vspace{-0.2in} 
  \end{center}
\end{wrapfigure}
To further quantitatively investigate the impact of OOD samples on the performance of OOD detection, in~\figurename~\ref{fig:motivation_ood}, we include the performance of OOD detection with a varied number of OOD samples from $\mathcal{D}^{out}=\mathcal{N}(2,1/2)$ (See Appendix~\ref{sec:data_detail} for the detailed experimental setting). The result shows that even with a few OOD samples, our algorithm can drastically reduce the FPR when compared to the detection algorithm that only depends on ID samples.

\begin{algorithm}[tb]
   \caption{Non-Parametric Test Time Adaptation for Out-Of-Distribution Detection}
   \label{alg:main}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} ID dataset ${D}^{in}$, a pretrained encoder $h_\theta$ with parameter $\theta$. Test sample $x_{o}$, threshold $\lambda$, $k$ for KNN selection. OOD selection margin $\gamma$ and  sample scale $\kappa$.
   \STATE {\bfseries Initialize} the memory bank with scales $\mathcal{M}=\{z_i:=h_\theta(x_i)/\parallel h_\theta(x_{i}) \parallel_2, s_i:=1\}_{x_i\in {D}^{in}}$.
   \STATE {\color{brown}\bfseries Inference stage for $x_{o}$.}
   
    \STATE  $z_{o}=h_\theta(x_{o})/\parallel h_\theta(x_{o}) \parallel_2$. \textit{// Normalize the feature.} \\
    \STATE $B=\left((z_{(1)},s_{(1)}),...,(z_{k)},s_{(k)})\right)$. \textit{// Search for nearest neighbors of the test feature.}  \\
    \STATE $S(x_o)=\frac{1}{k}\sum_{i=1}^k -\parallel z_o-z_{(i)} \parallel*s_{(i)}$ \textit{// Score.}
    \STATE  $\mathbf{1}\{S(x_o)\geq \lambda\}$ \textit{//Make OOD detection decision.} \label{alg1:decision}
   \STATE {\color{brown}\bfseries Memory augmentation for $x_{o}$.} 
   \IF{$S(x_o)< \lambda * \gamma$ } 
   \STATE $\mathcal{M}=\mathcal{M}\bigcup (z_o, \kappa)$ \textit{// Reliable OOD instance.}
   \ENDIF
   \IF{$S(x_o)> \lambda / \gamma$}
   \STATE $\mathcal{M}=\mathcal{M}\bigcup (z_o, 1)$ \textit{ // Reliable ID instance.}
   \ENDIF
\end{algorithmic}
\end{algorithm}

% {\color{cyan}
% \section{Methods}
% $$p_{\mathrm{in}}(x)\le \lambda_{\mathrm{in}}$$
% $$p_{\mathrm{in}}(x)\le \lambda_{\mathrm{in}} \textrm{ or }p_{\mathrm{out}}(x)\ge \lambda_{\mathrm{out}}$$
% $$p_{\mathrm{in}}(x) - p_{\mathrm{out}}(x)\le  \lambda_{\mathrm{in}} - \lambda_{\mathrm{out}}$$
% $$\frac{k_1}{Nr^{d-1}} - \frac{k_2}{nr^{d-1}}\le  \lambda_{\mathrm{in}} - \lambda_{\mathrm{out}}$$
% $$\frac{k_1}{k} - \frac{N}{n}\frac{k_2}{k}\le  \frac{Nr^{d-1}}{k}(\lambda_{\mathrm{in}} - \lambda_{\mathrm{out}})$$

% A.1  We have a score function $s(x)$ and monotonic function $f$ such that $f(s(x)) = p(x)$.

% A.2 There exists a nonzero measure space $\mathcal{X}$ such that $p_{\mathrm{in}}(x) = 0$ and $p_{\mathrm{out}}(x)>0$.
% }
% \section{Methods}



\vspace{-0.1cm}
\subsection{Non-Parametric Test Time Adaptation for Out-Of-Distribution Detection}
\vspace{-0.1cm}
% \textbf{Background: Out-of-Distribution Detection with Deep Nearest Neighbors~\cite{sun2022out}.} $k$-nearest neighbor is a kind of distance-based method, which leverages features embedding distances to classify ID and OOD samples. Specifically,\cite{sun2022out}
Here we describe \abbr and discuss its key merits compared to existing OOD detectors.

% Deep Nearest Neighbors~\cite{sun2022out} is a kind of distance-based method, which leverages features embedding distances to detect OOD samples. Compared to parametric density estimation methods~\cite{lee2018simple} that regards the feature space as a mixture of multivariate Gaussian distributions, KNN owns the following main advantages~\cite{sun2022out}: (1) KNN does not impose strong distributional assumption like the mixture of Gaussians assumption; (2) KNN can be fast even when the database contains billions of images~\cite{johnson2019billion} compared to Mahalanobis distance~\cite{lee2018simple} that  needs to computes the inverse of the covariance matrix. (3) The algorithm can be applied to various backbones and agnostic to training algorithms.

K Nearest Neighbors (KNN)~\cite{sun2022out} is a distance-based OOD detection method, which utilizes feature embedding to compute distances and detect OOD samples. Compared to parametric density estimation methods, KNN is advantageous in that it does not impose strong distributional assumptions, and is efficient for large databases with billions of images. The proposed \abbr improves KNN~\cite{sun2022out} by \textbf{explicitly exploiting online test samples that are detected as OOD}. The full detail of \abbr is given in Algorithm~\ref{alg:main}. For a given test sample $x_o$, we first find its $k$ nearest neighbors in the memory bank $\mathcal{M}$, which is initialized from the normalized training features, and the scale $s_i$ of all ID samples are set to $1$. We then calculate the score $S(x_o)$ as the negative of the average weighted distance of $k$-nearest neighbors $\frac{1}{k}\sum_{i=1}^k -\parallel z_o-z_{(i)} \parallel*s_{(i)}$. The threshold $\lambda$ is chosen so that a high fraction of the ID validation data ($95\%$) can be correctly classified. The core component of \abbr is the memory augmentation in Algorithm~\ref{alg:main}, as explained in full detail below.

(1) \textbf{OOD/ID sample selection.} 
Using all online samples to augment the $\mathcal{M}$ is not desirable, as they add noise to the memory bank and may deteriorate performance. To avoid this issue, we use a selection margin $\gamma\geq 1$ to filter unreliable OOD samples. Only if the score of $x$ is smaller than $\gamma*\lambda$, it will be a reliably detected OOD sample. Similarly, only if the score is higher than $\gamma/\lambda$, it will be a reliable ID sample.
(2) \textbf{Highlight the contribution of detected OOD samples.} Recall that our objective is to assign smaller scores to OOD samples than ID samples. However, given $x_o\in\mathcal{D}^{out}$, if its $k$-nearest neighbors are all OOD samples, they are highly similar and $-\parallel z_o-z_{i}\parallel$ will be large (small in magnitude), which is opposite to our goal. We thus introduce a large scale $\kappa\geq 1$ for reliably detected OOD samples to highlight their contributions\footnote{To illustrate the importance of OOD scale $\kappa$, we assume $\lambda=-1.0$ and $k=1$. Given $x_o=[2,2]\in\mathcal{D}^{out}$ and $\mathcal{M}=\{([1,1],1), ([0,0],1)\}$, we get $S(x_o)=-1.4$. If $\mathcal{M}$ contains an OOD sample $([2.5,2.5],\kappa)$, we hope $x_o$ with OOD neighbors has a low score. In this case, the score is $-0.707\kappa$. If $\kappa=1$, then $S(x_o)$ increases from $-1.4$ to $-0.7$ and will be identified as ID. We hence need a scale greater than $1$ to correct this phenomenon. $\kappa\rightarrow \infty$ means that once the $k$-nearest neighbors of $x_o$ contain OOD samples, then $x_o$ will be identified as OOD.
}.  (3) \textbf{Non-parametric adaptation}. After choosing reliably detected OOD samples and assigning them an appropriate scale, we augment the memory bank by including the selected feature vectors, i.e. $\mathcal{M}=\mathcal{M}\bigcup (z_o, \kappa)$. In contrast, existing TTA methods~\cite{sun2020test,zhang2021test,sun2020test,zhang2022domain} require additional training or fine-tuning to extract information from the detected OOD samples into models, leading to more computational overheads and making them less suitable for an online setting.

% \textbf{The relation between Algorithm~\ref{alg:main} and dynamic decision boundary in the motivating example.} In the latter, we show that Algorithm~\ref{alg:main} partitions the score function into two parts, namely, $S^{in}$ and $S^{out}$ that dependent on ID neighbors and OOD neighbors respectively. Unlike previous methods that use $S^{in}$ and a fixed boundary, \abbr adjusts the boundary by the score from the estimated OOD information.
\vspace{-0.15cm}
\subsection{Theoretical justification}
% The benefits of the proposed algorithm and how we derive it is theoretically detailed in this subsection.
\vspace{-0.15cm}
\subsubsection{Log conditional
densities score function.}\label{sec:log}
\vspace{-0.15cm}
To study how OOD samples influence the detection process, we partition the score function into two components, one dependent only on ID neighbors and the other dependent on OOD neighbors. We show that unlike previous methods that use ID neighbors and a fixed boundary, \abbr adjusts the boundary by the score from the estimated OOD information and prefers a lower false positive rate. Without access to OOD distribution, the typical decision rule is 
\vspace{-0.1cm}
\begin{align}
\mathbf{I}\{S(x|\mathcal{D}^{in})\geq \lambda\},\label{eq:xue:0}
\end{align}
where $\mathcal{D}^{in}$ is the ID sample set. We treat samples with scores higher than $\lambda$ as ID. The potential drawback is that the value of $\lambda$ is typically relatively small so that the in-distribution detection maintains enough accuracy. If we can access the estimated OOD distribution information, we may use a combined decision rule as follow:
\begin{align}
\mathbf{I}\{S(x|\mathcal{D}^{in}, \hat{\mathcal{D}}^{out})\ge \lambda\},\label{eq:xue:1}
\end{align}
where $\hat{\mathcal{D}}^{out}$ is the estimated OOD sample set. Intuitively, people usually hope the score function shows similar behavior as the probability function of ID, i.e., the higher score means a higher chance/probability that the test sample $x$ is from ID. Therefore, one of the ideal choices is to set the score function being proportional to log probability, i.e., $$S(x|\mathcal{D}^{in},\hat{\mathcal{D}}^{out}) \propto \log \mathbbm{P}(x\textrm{ from ID}|\mathcal{D}^{in},\hat{\mathcal{D}}^{out}).$$
we obtain the following equation through the maximum likelihood estimator analysis, 
\begin{align}
\small
S(x|\mathcal{D}^{in},\hat{\mathcal{D}}^{out})\propto \underbrace{\sum_{x_i\in\mathcal{D}^{in}}\log p^{in}(x|x_i)}_{(a)} + \underbrace{\sum_{x_j\in\hat{\mathcal{D}}^{out}}\log p^{out}(x|x_j)}_{(b)},\label{eq:xue:3}
\vspace{-0.1cm}
\end{align}
where $p^{in}(\cdot)$ and $p^{out}(\cdot)$ are the conditional density/mass function of ID given a reference sample from ID and estimated OOD, respectively. We must address $p^{out}$ \textbf{is not} the probability of a sample  belonging to out-of-distribution, it is the conditional probability that a sample \textit{belonging to in-distribution} given a reference sample from the estimated OOD.

 % In a typical OOD detection setting, the in-distirbution sample $N$ is much larger than the test sample size $n$. When conducting the KNN selection for the density overlapping regime, we may have a very high chance to select more in-distirbution samples. If we directly compute the log probabilities in \eqref{eq:xue:3} with all $\lambda_{in} =\lambda_{out}$, we will highly overestimate the ID density. Thus it is necessary to introduce extra coefficients to balance influence of sampling when compute the log probabilities in \eqref{eq:xue:3}.

\begin{wrapfigure}{r}{0.245\textwidth}
  \begin{center}
  \advance\leftskip+1mm
    \vspace{-0.2in}  
    \includegraphics[width=0.24\textwidth]{imgs/motivation.pdf}
    \vspace{-0.2in} 
    \caption{\small $\mathcal{D}^{out}=\mathcal{N}(10,1/2)$.}
        \label{fig:motivation1}
    \vspace{-0.2in} 
  \end{center}
\end{wrapfigure}

The formulation \eqref{eq:xue:3} uses the sum of logarithmic conditional densities to detect OOD samples. Compared to the detection rule \eqref{eq:xue:0}, the detection rule \eqref{eq:xue:3} has more chance to successfully detect samples as OOD. The ID conditional density $p^{in}$ or $p^{out}$ is small (for example, far from the ID samples or near the estimated OOD samples), and we assign the OOD label to the sample because the log probability will be small enough. We use two scenarios in~\figurename~\ref{fig:motivation} to show the rationality of the decision rule \eqref{eq:xue:3}. 

% Because the probability is a value within $[0,1]$, a higher probability yields a larger negative log probability.
%One may expect that $p^{in}(x|x_i)$ increases when $x_i$ converging to $x$ and $p^{out}(x|x_j)$ decreases when $x_j$ converging to $x$. 


% Via the assumption A.1, the \eqref{eq:xue:1} is equivalent to 
% \begin{align}
% \mathbf{I}\{p_{in}(x|\mathcal{D}_{KNN}^{in}) \cdot p_{in}(x|\mathcal{D}_{KNN}^{out})\leq P_{in}\},\label{eq:xue:2}
% \end{align}
% where $p_{in}$ and $p_{out}$ are density functions, and $ P_{in},  P_{out}$ are crossponding thresholds to $\lambda_{in},\lambda_{out}$. The above decision rule involves two hyperparameters and we may use the log-ratio decision rule as a relaxation:
% \begin{align}
% &\mathbf{I}\left\{\log \left(\frac{p_{in}(x)}{p_{out}(x)}\right)\leq P\right\}\notag\\
% \Leftrightarrow&\mathbf{I}\left\{\log p_{in}(x) - \log p_{out}(x)\leq P\right\}\label{eq:xue:3}
% \end{align}
% When setting $P = \log(P_{in}/P_{out})$, we may directly view \eqref{eq:xue:2} as  adding inequality $-\log p_{out}(x)\le -\log P_{out}$ to $\log p_{in}(x)\le \log P_{in}$. 

\textit{Well separated ID/OOD in~\figurename~\ref{fig:motivation1}.} In this scenario, when the term $(a)$ in \eqref{eq:xue:3} is large enough (i.e., $x$ in a high-density distribution of ID, the density of OOD at $x$ must be very small, then $\log p^{out}\approx 0$. In this case, the decision rule reduces to the classic detection rule \eqref{eq:xue:0}. On the other hand, when $x$ is from OOD, both $(a)$ and $(b)$ are expected to be small, and we can safely assign the OOD label while sacrificing minimal ID accuracy.

\textit{Overlapped ID/OOD in~\figurename~\ref{fig:motivation2}.} In this setting, we consider the ID/OOD overlap in some high-density regimes. The classic OOD detection rule \eqref{eq:xue:0} has a small threshold $\lambda$ and can lead to a large number of OOD samples being classified as ID samples. When applying the detection rule \eqref{eq:xue:3}, we measure the conditional density given both ID/estimated OOD sample sets. As long as one of the terms $(a)$ or $(b)$ is small enough, which corresponds to the situations where $x$ is far from the ID reference samples or has enough close estimated OOD reference samples, we can still assign the sample $x$ with the OOD label. Our method, hence, yields a lower false positive rate.
\vspace{-0.1cm}
\subsubsection{Nonparametric density estimator}
\vspace{-0.1cm}
Until now, how to estimate the local density and OOD sample set in \eqref{eq:xue:3} remains unclear. In this subsection, we apply KNN to approximate local densities~\cite{zhao2022analysis} and derive our decision rule. In section~\ref{sec:ood_sample}  we show how to estimate the OOD sample set.
% In test time, we assume the sample is generated from a mixed distribution $P_{test}$ defined as 
% \begin{align}
% \mathcal{P}_{test} = \kappa \mathcal{P}_{in}  + (1-\kappa)\mathcal{P}_{out},
% \end{align}
% where $\kappa\in [0,1]$ and $\mathcal{P}_{in}$ and $\mathcal{P}_{out}$ are the marginal distribution of input images. We define $\mathcal{D}_{x}^{in} = \{x_i\}_{i=1}^N$ and $\mathcal{D}_{x}^{test} = \{x_i\}_{i=N+1}^{n+N}$ as the sample sets corresponding to the training and test stages respectively. Moreover, we assume the training and test stage have $N$ and $n$ sample sizes, respectively. 

To facilitate our discussion, we first consider an artificial setting in that we know the true in/out label of the test samples, and every sample is normalized by its $l_2$ norm to project the representation onto the unit sphere. For a given test sample $x$, we first use cosine similarity to collect the $k$ closet samples from $x$ as $\mathcal{D}_{KNN}(x)$ from $\mathcal{D}^{in}\cup \mathcal{D}^{test}$, where $\mathcal{D}^{test}$ is test time sample set that follows some mixed distribution of ID/OOD. Without loss of generality, we assume $\mathcal{D}_{KNN}(x)$ to contain $k_1$ and $k_2$ samples from ID/OOD, respectively. We denote two disjoint datasets $\mathcal{D}_{KNN}^{in}(x)$ and $\mathcal{D}_{KNN}^{out}(x)$ containing the ID/OOD samples in $\mathcal{D}_{KNN}(x)$. Next, we make an assumption on the conditional densities $p^{in}(x|x_i)$ and $p^{out}(x|x_j)$ as follows:


{\it Assumption 1:} There exist two positive constants $\lambda_{in} <\lambda_{out}$ such that $p^{in}(x|x_i)$ and $p^{out}(x|x_j)$ are proportional to $\exp(-\lambda_{in}\|x-x_i\|_2)$ and $\exp(-\lambda_{out}\|x-x_j\|_2)$.\footnote{Here we assume the density function's tails performance is exponential. Via more sophisticated analysis, we may further relax the density being subgaussian/subexponential.}

 We use $\lambda_{in}$ and $\lambda_{out}$ to describe the influence of ID and OOD samples. Let us consider a sample $x$ and a reference point $y$ that is close to $x$. 
 Intuitively, one may expect that $x$ has a higher chance of being an ID sample if $y$ is an ID sample and a lower chance if $y$ is believed from OOD. In other words, for the same reference sample $y$, we should have $p^{in}(x|y)> p^{out}(x|y)$, which is achieved by setting $\lambda_{in}<\lambda_{out}$ in {\it Assumption 1}. During the testing stage, we can hardly ensure $y$ being from OOD with probability $1$. Therefore, it would be safer to treat $y$ as a reference sample that contributes less than a normal ID reference sample in accessing the chance that the sample $x$ is ID.\footnote{If the exact OOD sample set is available in the test stage, the OOD detection task fall into the semi-supervised learning field, and we may use the log-liklihood-ratio~\cite{kawakita2013semi} as a score function, that is, $S(x|\mathcal{D}^{in},\hat{\mathcal{D}}^{out}) \propto \log \left({\mathbbm{P}(x\textrm{ from ID}|\mathcal{D}^{in})}/{\mathbbm{P}(x\textrm{ from OOD}|\mathcal{D}^{out})}\right) %= \log \mathbbm{P}(x\textrm{ from ID}|\mathcal{D}^{in}) - \log \mathbbm{P}(x\textrm{ from OOD}|\mathcal{D}^{out})$.} 
 $.} We then combine {\it Assumption 1} with $\mathcal{D}^{in}_{KNN}(x)$ and $\mathcal{D}^{out}_{KNN}(x)$ instead of $\mathcal{D}^{in}$ and $\hat{\mathcal{D}}^{out}$ in terms of $(a)$ and $(b)$.  
\vspace{-0.1cm}
\begin{align}
\small
&(a)\propto - \sum_{x_i\in\mathcal{D}^{in}_{KNN}(x)}\lambda_{in}\|x-x_i\|_2\notag \\
&(b)\propto - \sum_{x_i\in\mathcal{D}^{out}_{KNN}(x)}\lambda_{out}\|x-x_i\|_2\notag\\
\Rightarrow& (a) + (b) \propto -\sum_{x_i\in\mathcal{D}_{KNN}(x)}\|x-x_i\|_2\cdot s(x_i)\label{eq:xue:4}
\end{align}
where we set $s(x_j) = 1$ if $x_j$ is from ID and $s(x_j) = \lambda_{out}/\lambda_{in}$ otherwise. Finally combine \eqref{eq:xue:4} with \eqref{eq:xue:3} and we end up with the decision rule used in {\bf Algorithm~\ref{alg1:decision} line 7}:
\vspace{-0.1cm}
\begin{equation}
\begin{aligned}
\mathbf{I}\left\{-\sum_{x_j\in\mathcal{D}_{KNN}} \|x-x_j\|_2 \cdot s(x_j) \ge \lambda\right\}\label{eq:xue:5}
\end{aligned}  
\end{equation}

\vspace{-0.1cm}
Note that in the detection rule \eqref{eq:xue:5}, we require knowledge on the distribution labels for all samples in $\mathcal{D}_{KNN}$, which is inaccessible for samples from $\mathcal{D}_{test}$ in practice. In this paper, we instead propose an estimation of distribution labels via \eqref{eq:xue:5} with a slightly larger $\lambda$. Since usually the ID sample size $N$ is much larger than the test sample size $n$, detecting extra ID samples only leads to marginal improvement. We may directly use $\mathcal{D}^{in}$ instead of all ID samples. 

\subsubsection{Estimation of OOD sample set.}\label{sec:ood_sample}
Next, we consider the estimation of the OOD sample set. Let denote $\mathcal{D}_{KNN}^{out,T}$ and $\mathcal{D}_{KNN}^{out,F}$ as the disjoint sample sets containing the true OOD sample and false OOD sample in $\mathcal{D}_{KNN}^{out}$. We will have the following separation:
\begin{equation}
\begin{aligned}
\tiny
&-\sum_{x_j\in\mathcal{D}_{KNN}} s(x_j)\|x-x_j\|_2= \\
&-\sum_{x_j\in\mathcal{D}_{KNN}^{out,T}(x)}s(x_j)\|x-x_j\|_2 
-\sum_{x_j\in\mathcal{D}_{KNN}^{out,F}(x)}s(x_j)\|x-x_j\|_2
\end{aligned}
\end{equation}
If we overestimated the OOD sample size by a margin, the corresponding $\sum_{x_j\in \mathcal{D}_{KNN}^{out}(x)}\|x-x_j\|_2s(x_j)$ will be overestimated and yield a lower AUC on ID/OOD detection. On the other hand, if we only collect the OOD sample with enough confidence (e.g., the small enough value from the score function), the corresponding $\sum_{x_j\in \mathcal{D}_{KNN}^{out}(x)}\|x-x_j\|_2s(x_j)$ becomes smaller and the decision rule of \eqref{eq:xue:5} leans more on the high confidence ID samples. In the extreme case, the $\mathcal{D}_{KNN}^{out}(x)$ being empty set, the $\sum_{x_j\in \mathcal{D}_{KNN}^{out}(x)}\|x-x_j\|_2s(x_j)$ becomes 0 and the detection rule \eqref{eq:xue:5} reduces to the classic detection rule \eqref{eq:xue:0}. Therefore, only keeping the test sample with high confidence, as the detected OOD sample is safer. In this paper, we propose to use the following decision rule to collect the estimated OOD samples during the test stage ({\bf Algorithm~\ref{alg1:decision} line 9}):
\begin{align}
\mathbf{I}\left\{S(x_0|\mathcal{D}^{in}_{KNN}(x),\hat{\mathcal{D}}^{out}_{KNN}(x))<\lambda\cdot \gamma\right\},
\end{align}
where $\gamma\ge 1$ and $\hat{\mathcal{D}}^{out}_{KNN}(x)$ is the estimated OOD sample set and is empty at the beginning.

% where $n_1$ is the ID sample size in test dataset $\mathcal{D}_{x,test}$, and $s(x,x_j)$ is defined as follow:
% \begin{align}
% s(x,x_j) = \langle x,x_j\rangle = 1-\frac{1}{2}\left\|x-x_j\right\|_2^2.
% \end{align}
%  The probability part then becomes
% \begin{align}
% \hat{p}_{in}(x) &= \frac{1}{N+n_1} \left(k_1 -\frac{1}{2}\sum_{j=1}^{k_1}\|x-x_j\|_2^2\right)\notag\\
% \hat{p}_{out}(x) &= \frac{1}{n-n_1} \left(k-k_1 -\frac{1}{2}\sum_{j=k_1+1}^{k}\|x-x_j\|_2^2\right)\notag.
% \end{align}
% We now consider the estimated probability difference.
% \begin{align}
% &\hat{p}_{in}(x) - \hat{p}_{out}(x)\notag\\
% =&\frac{1}{N+n_1} \left(k_1 -\frac{1}{2}\sum_{j=1}^{k_1}\|x-x_j\|_2^2\right)\notag\\
% -& \frac{1}{n-n_1} \left(k-k_1 -\frac{1}{2}\sum_{j=k_1+1}^{k}\|x-x_j\|_2^2\right)\notag\\
% =&\frac{k}{2(N+n_1)}\left[\left(\frac{2k_1}{k} -\frac{1}{k}\sum_{j=1}^{k_1}\|x-x_j\|_2^2\right)\right.\notag\\
% -&\left.\frac{N+n_1}{n-n_1}\left(\frac{2(k-k_1)}{k} -\frac{1}{k}\sum_{j=k_1+1}^{k}\|x-x_j\|_2^2\right)\right]\notag\\
% =&\frac{k}{2(N+n_1)}\left(\frac{2k_1}{k} -\frac{N+n_1}{n-n_1}\frac{2(k-k_1)}{k}\right)\\
% =&\frac{k}{2(N+n_1)}\left[\left(\frac{2k_1}{k} -\frac{1}{k}\sum_{j=1}^{k_1}\|x-x_j\|_2^2\right)\right.\notag\\
% -&\left.\frac{N+n_1}{n-n_1}\left(\frac{2(k-k_1)}{k} -\frac{1}{k}\sum_{j=k_1+1}^{k}\|x-x_j\|_2^2\right)\right]\notag\\
% =&\phi_0\frac{1}{k}\sum_{j=1}^{k}\left(\frac{1}{2}-\|x-x_j\|_2^2\right)\cdot w_{j}\notag,
% % -&\left.\frac{N+n_1}{n-n_1}\left(\frac{2(k-k_1)}{k} -\frac{1}{k}\sum_{j=k_1+1}^{k}\|x-x_j\|_2^2\right)\right]\notag\\
% \end{align}
% where $\phi_0 = \frac{k}{2(N+n_1)}$, $w_j = 1$ for ID samples and $w_j = \phi_1 = -\frac{N+n_1}{n-n_1}$ for OOD samples. In practice, we usually have $N\gg n> n_1$ and $n_1 = \mathcal{O}(\kappa n)$, $\phi_0 \approx \frac{k}{N}$  being a constant independent on test sample size, and $\phi_1\approx \frac{N}{(1-\kappa)n}=\mathcal{O}\left(\frac{N}{n}\right)$






% , we go along this line and detection rule \eqref{eq:xue:3} becomes:
% \begin{align}
% \mathbf{I}(\frac{1}{N}\sum_{\|x_0-x\|\le r})
% \end{align}








==> sections/exp_icml.tex <==


\begin{table*}[]
\caption{\textbf{Results on small benchmarks}, where the ID dataset is CIFAR-10. All methods are based on a model trained on ID data. $\uparrow$ indicates larger values are better and vice versa.} \label{tab:cifar}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{\textbf{SVHN}} & \multicolumn{2}{c}{\textbf{LSUN}} & \multicolumn{2}{c}{\textbf{iSUN}} & \multicolumn{2}{c}{\textbf{Texture}} & \multicolumn{2}{c}{\textbf{Place365}} & \multicolumn{2}{c}{\textbf{Average}} \\
\multicolumn{1}{c}{} & \textbf{FPR $\downarrow$} & \textbf{AUROC $\uparrow$} & \textbf{FPR $\downarrow$} & \textbf{AUROC $\uparrow$} & \textbf{FPR $\downarrow$} & \textbf{AUROC $\uparrow$} & \textbf{FPR $\downarrow$} & \textbf{AUROC $\uparrow$} & \textbf{FPR $\downarrow$} & \textbf{AUROC $\uparrow$} & \textbf{FPR $\downarrow$} & \textbf{AUROC $\uparrow$} \\
\midrule
\multicolumn{13}{c}{\textbf{Without Contrastive Learning}} \\
MSP & 59.66 & 91.25 & 45.21 & 93.80 & 54.57 & 92.12 & 66.45 & 88.50 & 62.46 & 88.64 & 57.67 & 90.86 \\
ODIN & 20.93 & 95.55 & 7.26 & 98.53 & 33.17 & 94.65 & 56.40 & 86.21 & 63.04 & 86.57 & 36.16 & 92.30 \\
Energy & 54.41 & 91.22 & 10.19 & 98.05 & 27.52 & 95.59 & 55.23 & 89.37 & 42.77 & 91.02 & 38.02 & 93.05 \\
GODIN & 15.51 & 96.60 & 4.90 & 99.07 & 34.03 & 94.94 & 46.91 & 89.69 & 62.63 & 87.31 & 32.80 & 93.52 \\
Mahalanobis & 9.24 & 97.80 & 67.73 & 73.61 & 6.02 & 98.63 & 23.21 & 92.91 & 83.50 & 69.56 & 37.94 & 86.50 \\
KNN & 24.53 & 95.96 & 25.29 & 95.69 & 25.55 & 95.26 & 27.57 & 94.71 & 50.90 & 89.14 & 30.77 & 94.15 \\ \Gray
\abbr & \textbf{2.17} & \textbf{99.35} & \textbf{5.80} & \textbf{98.90} & \textbf{4.90} & \textbf{98.89} & \textbf{15.82} & \textbf{96.74} & \textbf{7.50} & \textbf{97.31} & \textbf{7.24} & \textbf{98.24} \\ \midrule
\multicolumn{13}{c}{\textbf{With Contrastive Learning}} \\
CSI & 37.38 & 94.69 & 5.88 & 98.86 & 10.36 & 98.01 & 28.85 & 94.87 & 38.31 & 93.04 & 24.16 & 95.86 \\
SSD+ & 1.51 & 99.68 & 6.09 & 98.48 & 33.60 & 95.16 & 12.98 & 97.70 & 28.41 & 94.72 & 16.52 & 97.15 \\
KNN & 2.42 & 99.52 & 1.78 & 99.48 & 20.06 & 96.74 & 8.09 & 98.56 & 23.02 & 95.36 & 11.07 & 97.93 \\ \Gray
\abbr & \textbf{1.79} & \textbf{99.71} & \textbf{1.79} & \textbf{99.67} & \textbf{6.81} & \textbf{98.97} & \textbf{6.97} & \textbf{98.92} & \textbf{10.19} & \textbf{97.53} & \textbf{5.51} & \textbf{98.96} \\ \bottomrule
\end{tabular}%
}
\end{table*}

\begin{table*}[]
\centering
\caption{\textbf{Results on hard OOD detection tasks}, where the ID dataset is CIFAR-10. All methods are based on a model trained by supervised contrastive loss. $\uparrow$ indicates larger values are better.} \label{tab:cifar_hard}
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{ccccccccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{\textbf{LSUN-FIX}} & \multicolumn{2}{c}{\textbf{ImageNet-FIX}} & \multicolumn{2}{c}{\textbf{ImageNet-Resize}} & \multicolumn{2}{c}{\textbf{CIFAR-100}} & \multicolumn{2}{c}{\textbf{Avg}} \\
 &  \textbf{FPR $\downarrow$} & \textbf{AUROC $\uparrow$} & \textbf{FPR $\downarrow$} & \textbf{AUROC $\uparrow$} & \textbf{FPR $\downarrow$} & \textbf{AUROC $\uparrow$} & \textbf{FPR $\downarrow$} & \textbf{AUROC $\uparrow$} & \textbf{FPR $\downarrow$} & \textbf{AUROC $\uparrow$} \\ \midrule
SSD+ & 29.86 & 94.62 & 23.26 & 93.19 & 45.62 & 89.72 & 45.50 & 87.34 & 36.06 & 91.22 \\
KNN & 21.52 & 96.51 & 25.92 & 95.71 & 30.16 & 95.08 & 38.83 & 92.75 & 29.11 & 95.01 \\ \Gray
\abbr & \textbf{12.04} & \textbf{98.16} & \textbf{22.81} & \textbf{96.45} & \textbf{12.48} & \textbf{97.75} & \textbf{34.73} & \textbf{93.46} & \textbf{20.52} & \textbf{96.46} \\ \bottomrule
\end{tabular}%
}
\end{table*}

In this section, we show that (1) \abbr attains superior performances on small and large-scale benchmarks; (2) we design several strong TTA baselines, which are all shown be inferior to \abbr; (3) \abbr performs well under different OOD detection settings, and (4) how to select the best hyper-parameters for different benchmarks.

\textbf{Benchmarks.} We study OOD detection on the following two settings: (1) \textbf{Small Benchmarks that are routinely used.} We use $50,000$  training  images  and  $10,000$ test images of the CIFAR benchmarks for model training. The model is evaluate on common OOD datasets: Textures~\cite{cimpoi2014describing}, SVHN~\cite{netzer2011reading}, LSUN~\cite{yu2015lsun}, Places365~\cite{zhou2017places}, Textures~\cite{cimpoi2014describing}, and iSUN~\cite{xu2015turkergaze} and more chanllenging OOD datasets: LSUN-FIX~\cite{yu2015lsun}, ImageNet-FIX~\cite{deng2009imagenet}, ImageNet-Resize~\cite{deng2009imagenet}, and CIFAR-100.  (2) \textbf{Large-scale ImageNet Task~\cite{huang2021mos}} that contains a widespread range of domains such as fine-grained images, scene images, and textural images. The ImageNet~\cite{deng2009imagenet} training model is evaluated on four OOD datasets: Places365~\cite{zhou2017places}, Textures~\cite{cimpoi2014describing}, iNaturalist~\cite{van2018inaturalist}, and SUN~\cite{xiao2010sun}. (3) \textbf{Other evaluation settings}. We evaluate \abbr under different test distributions, such as (a) OOD samples are from different OOD distributions sequentially, namely, the algorithm is evaluated and adaptated on a series of OOD datasets; (b) the test OOD distribution is a mixture of multiple OOD distributions rather than coming from the same distribution; (c) the test distribution is a mixture of ID and OOD distributions.

\textbf{Baselines.} We incorporate several baselines that derive OOD scores from a model trained with common softmax cross-entropy (CE) loss, such as MSP~\cite{hendrycks2016baseline}, ODIN~\cite{liang2018enhancing}, Mahalanobis~\cite{lee2018simple}, Energy~\cite{liu2020energy}, GODIN~\cite{hsu2020generalized}, KNN~\cite{sun2022out}. Besides, there are several baselines that benefit from contrastive learning, such as CSI~\cite{tack2020csi}, SSD+~\cite{sehwag2021ssd}, and KNN~\cite{sun2022out}.

\textbf{Evaluation metrics} include (1) the false positive rate (FPR95) of OOD samples when the true positive rate of ID is at $95\%$. (2) the area under the receiver operating characteristic (AUROC), which tells us whether our model is able to correctly rank examples. (3) the inference time per image that is averaged from all test images in milliseconds. See Appendix \ref{sec:data_detail} for more information, including baselines, hyper-parameters details, and implementation details.

\subsection{Evaluation and Ablations on Small Out-of-distribution Detection Benchmarks}

% \textbf{Experimental details.} For CIFAR-10, we use ResNet-18~\cite{he2016deep} as the backbone. We conduct two different settings considering the ID training process: (1) The training loss is cross-entropy loss, and the model is trained for 100 epochs. The learning rate is $0.1$ and decays at epochs $50,75,90$ respectivly by a factor $10$. (2) The training loss is supervised contrastive loss~\cite{khosla2020supervised} with temperature $\tau=0.1$. The total training epochs and batch size are set to $500, 1024$, respectively. All models are trained using stochastic gradient descent with momentum $0.9$ and weight decay $10^{-4}$. 

\textbf{Experimental details.} For CIFAR-10, we use ResNet-18~\cite{he2016deep} as the backbone. We conduct two different settings considering the ID training process: (1) The training loss is cross-entropy loss. (2) The training loss is supervised contrastive loss~\cite{khosla2020supervised} with temperature $\tau=0.1$.
\begin{table}[b]
\vspace{-0.3cm}
\caption{\textbf{FPR95 of TTA methods on small benchmarks}.}\label{tab:tta}
\centering
\small
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccc}
\toprule
 & SVHN & LSUN & iSUN & Texture & Avg & Inference time (ms) \\ \midrule
Energy & 54.41 & 10.19 & 27.52 & 55.23 & 36.84 & 4.81 \\
TTA Energy & 28.95 & 50.00 & 16.67 & 60.00 & 38.91 & 24.50 \\
Mahalanobis & 59.20 & 11.01 & 54.47 & 31.61 & 39.07 & 21.82 \\
TTA Mahalanobis & 50.00 & 18.42 & 39.28 & 27.64 & 33.84 & 50.98 \\
KNN & 24.53 & 25.29 & 25.55 & 27.57 & 25.74 & 4.97 \\
TTA KNN & 26.00 & 14.38 & 17.95 & 24.70 & 20.76 & 24.85 \\  \Gray
AdaODD & \textbf{2.17} & \textbf{5.80} & \textbf{4.90} & \textbf{15.82} & \textbf{7.17} & 5.84
\\ \bottomrule
\end{tabular}%
}
\end{table}
\textbf{\abbr beats all baselines by a large margin.} The results are shown in Table~\ref{tab:cifar}, where the proposed \abbr reduces the average FPR95 of previous best model from $\mathbf{30.77}$ to $\mathbf{7.24}$. Note that \abbr achieves superior results in large OOD datasets, such as the Places365~\cite{zhou2017places} dataset, where the best FPR95 of the baseline models is $\mathbf{42.77}$ but \abbr achieves $\mathbf{7.5}$. Taking into account the models trained by the loss of supervised contrast learning (SupCon), all methods, including CSI~\cite{tack2020csi}, SSD+~\cite{sehwag2021ssd}, and KNN~\cite{sun2022out} achieve superior results compared to models trained by cross-entropy loss. The proposed nonparametric test-time adaptation method is agnostic to the training procedure and is compatible with models trained under different losses. Table~\ref{tab:cifar} shows that the FPR95 of \abbr with SupCon loss ($\mathbf{5.51}$) is only half of the previous best result ($\mathbf{11.07}$). 

\textbf{\abbr beats strong TTA baselines.} We modify several baselines into TTA by proposing some specific training strategies during test. In particular, given a detected OOD sample $x_{out}$ and a set of ID samples $x_{in}\sim\mathcal{D}_{in}$, we add the following training loss during inference as follows (1) \textbf{TTA Energy~\cite{liu2020energy}}: $L_{energy}=\max(0,E(x_{in}-m_{in}))^2+\max(0,m_{out}-E(x_{out}))^2$, where $m_{out}$ is the separate margin hyperparameter for the two squared hinge loss and $E$ is the energy function. Namely, we penalize the out-of-distribution samples with energy lower than the margin parameter $m_{out}$. The  $m_{in}$ is chosen from $[-3, -5, -7]$ and $m_{out}$ is chosen from $[-15,-19,-23,-27]$ as~\cite{liu2020energy}. (2) \textbf{TTA Mahalanobis~\cite{lee2018simple}}, and \textbf{TTA KNN~\cite{sun2022out}}. We use metric learning to enlarge the margin between ID and OOD representations. Specifically, for the anchor sample $x_{out}$,we sample $x_{in}\sim\mathcal{D}_{in}$ as the negative sample, a random sampled $\bar{x}_{out}$ as the positive sample. Finally, we optimize the triplet loss $L_{tri}=\max(d(x_{out},\bar{x}_{out})-d(x_{out},x_{in})+m,0)$, where $m$ is the margin and $d$ is the distance (L-2 norm by default). The results in Table~\ref{tab:tta} demonstrate that all of the strong baselines designed are better than their offline counterparts, which confirms the significance of test time adaptation. However, they are still outperformed by \abbr. It is worth noting that all of these methods require retraining the model when an OOD sample is detected, resulting in computational burdens and limiting their practicality. Additionally, the experiments suggest that TTA is not always beneficial since during inference, the model is trained using only one data instance instead of a batch of data, which leads to highly noisy gradients that could potentially harm the model optimization process. 


\textbf{\abbr perform well on more challenging OOD tasks.} We follow \cite{sun2022out,tack2020csi} and evaluate \abbr on several hard OOD dataset: LSUN-FIX~\cite{yu2015lsun}, ImageNet-FIX~\cite{deng2009imagenet}, ImageNet-Resize~\cite{deng2009imagenet}, and CIFAR-100, where the OOD samples are particularly challenging to detect. Table~\ref{tab:cifar_hard} shows that even with models trained with SupCon loss, the baselines SSD+~\cite{sehwag2021ssd} and KNN~\cite{sun2022out} cannot achieve a low false positive rate as in Table~\ref{tab:cifar}, revealing the difficulty of the tasks. However, \abbr reduces the FPR95 by $\mathbf{15.58}$ and $\mathbf{8.59}$ compared to SSD+~\cite{sehwag2021ssd} and KNN~\cite{sun2022out} respectively.

\begin{table*}[]
\caption{\textbf{Results on large-scale benchmarks}, where the ID dataset is ImageNet. All methods are based on a model trained on ID data only. $\uparrow$ indicates larger values are better.} \label{tab:imagenet}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Inference \\ time (ms)\end{tabular}}} & \multicolumn{2}{c}{\textbf{iNaturalist}} & \multicolumn{2}{c}{\textbf{SUN}} & \multicolumn{2}{c}{\textbf{Places}} & \multicolumn{2}{c}{\textbf{Textures}} & \multicolumn{2}{c}{\textbf{Average}} \\ 
 & & \textbf{FPR $\downarrow$} & \textbf{AUROC $\uparrow$} & \textbf{FPR $\downarrow$} & \textbf{AUROC $\uparrow$} & \textbf{FPR $\downarrow$} & \textbf{AUROC $\uparrow$} & \textbf{FPR $\downarrow$} & \textbf{AUROC $\uparrow$} & \textbf{FPR $\downarrow$} & \textbf{AUROC $\uparrow$} \\ \midrule
MSP & 7.04 & 54.99 & 87.74 & 70.83 & 80.86 & 73.99 & 79.76 & 68.00 & 79.61 & 66.95 & 81.99 \\
ODIN & 7.05 & 47.66 & 89.66 & 60.15 & 84.59 & 67.89 & 81.78 & 50.23 & 85.62 & 56.48 & 85.41 \\
Energy & 7.04 & 55.72 & 89.95 & 59.26 & 85.89 & 64.92 & 82.86 & 53.72 & 85.99 & 58.41 & 86.17 \\
GODIN & 7.04 & 61.91 & 85.40 & 60.83 & 85.60 & 63.70 & 83.81 & 77.85 & 73.27 & 66.07 & 82.02 \\
Mahalanobis & 35.83 & 97.00 & 52.65 & 98.50 & 42.41 & 98.40 & 41.79 & 55.80 & 85.01 & 87.43 & 55.47 \\
KNN & 10.31 & 59.00 & 86.47 & 68.82 & 80.72 & 76.28 & 75.76 & 11.77 & 97.07 & 53.97 & 85.01 \\ \Gray
\abbr & 10.31 & \textbf{4.48} & \textbf{98.85} & \textbf{18.70} & \textbf{93.76} & \textbf{33.59} & \textbf{87.81} & \textbf{7.13} & \textbf{98.22} & \textbf{15.97} & \textbf{94.66} \\ \bottomrule
\end{tabular}%
}
\vspace{-0.6cm}
\end{table*}
\begin{figure}
\vspace{-0.5cm}
\centering
\begin{minipage}[t]{\textwidth}     
\subfigure[Reevaluation]
{\includegraphics[width=0.235\textwidth]{imgs/cifar_avg_in.pdf}
\label{fig:cifar_avg_in}
}
\subfigure[FPR]
{\includegraphics[width=0.235\textwidth]{imgs/cifar_avg_out.pdf}
\label{fig:cifar_avg_out}
}
\end{minipage}
\vspace{-0.2cm}
\caption{\textbf{Ablation of using $k$-avg, $k$-th, $k$-median nearest neighbor distance} considering different OOD datasets on small OOD detection benchmark.}\label{fig:cifar_avg}
\vspace{-0.2cm}
\end{figure}
\textbf{The effect of test-time adaptation for ID data.} One main concern is that as adaptation progresses, the ID samples will be harder to identify because more outliers are added to the memory bank and large scales are assigned. To address this concern, we reevaluate the adapted model in the ID samples, which can test whether the adapted model can still identify the ID examples successfully. For example, in~\figurename~\ref{fig:cifar_magina}, we first evaluate and adapt the algorithm to SVHN dataset. After the adaptation, we evaluate the adapted model on ID samples, namely using the augmented memory bank and calculate the score by $\frac{1}{k}\sum_{i=1}^k -\parallel z_o-z_{(i)} \parallel*s_{(i)}$ in Algorithm~\ref{alg:main}. The evaluation metric is termed \textbf{ID reevaluation accuracy}. To conclude, the results show that the adaptation process only slightly reduces the accuracy of the ID samples but achieves a significant benefit for the detection of the OOD samples compared to the non-adapted model, whose FPR95 is $30.28$. 


\textbf{How to choose the best $\gamma$ and $\kappa$?}  We study the effect of selection margin $\gamma$ and sample scale $\kappa$ in \figurename~\ref{fig:cifar_magin}. We observe that: (i) A selection margin $\gamma$ too small or too large leads to inferior OOD detection results (\figurename~\ref{fig:cifar_maginb}). The reason is that the small $\gamma$ brings many noisy samples that may not be OOD instances. Large $\gamma$ cannot utilize the benefit of test-time adaptation because only a small part OOD samples satisfy the condition, namely $score>\lambda*\gamma$. Hence, larger $\gamma$ attains inferior OOD detection results but retains better ID detection accuracy. (ii) A larger scale $\kappa$ always leads to a better OOD detection performance because all OOD samples are of large weight. In the extreme case, namely $\kappa=\infty$, given a test sample $x^*$, once there is an OOD sample in its $k$ nearest neighbors, $x^*$ will attain a very low score and be decided as an OOD sample. At the same time, using a large $\kappa$ leads to a worse ID detection performance (\figurename~\ref{fig:cifar_magina}). We choose $\kappa=1.5$ and $\gamma=5.0$ by default so that the adapted model retains a comparable ID detection accuracy to models without TTA.

\begin{figure*}[t]
\centering
\begin{minipage}[t]{\textwidth}        
\subfigure[Selection margin $\gamma$.]
{\includegraphics[width=0.25\textwidth]{imgs/cifar_svhn_in.pdf}
\label{fig:cifar_magina}
}
\subfigure[Sample scale $\kappa$.]
{\includegraphics[width=0.25\textwidth]{imgs/cifar_svhn_out.pdf}
\label{fig:cifar_maginb}
}
\subfigure[Reevaluation]
{\includegraphics[width=0.2\textwidth]{imgs/cifar_norm_in.pdf}
\label{fig:cifar_norm_in}
}
\subfigure[FPR]
{\includegraphics[width=0.2\textwidth]{imgs/cifar_norm_out.pdf}
\label{fig:cifar_norm_out}
}
\end{minipage}
\vspace{-0.4cm}
\caption{\textbf{Ablation studies of OOD selection margin $\gamma$ and sample scale $\kappa$}. (a) Reevaluation accuracy of ID samples and (b) FPR95 of OOD samples in the SVHN~\cite{netzer2011reading} dataset. (c,d) Ablation of the effect of using normalization vs. without normalization%(c) Reevaluation accuracy of ID samples and (d) FPR95 of OOD samples in the LSUN~\cite{yu2015lsun} dataset. }
}\label{fig:cifar_magin}\label{fig:cifar_norm}
\vspace{-0.3cm}
\end{figure*}

% \begin{figure}[t]
% \centering
% \begin{minipage}[t]{\textwidth}  
% \subfigure[ID reevaluation accuracy]
% {\includegraphics[width=0.22\textwidth]{imgs/cifar_norm_in.pdf}
% \label{fig:cifar_norm_in}
% }
% \subfigure[FPR]
% {\includegraphics[width=0.22\textwidth]{imgs/cifar_norm_out.pdf}
% \label{fig:cifar_norm_out}
% }
% % \subfigure[ID reevaluation accuracy]
% % {\includegraphics[width=0.22\textwidth]{imgs/cifar_avg_in.pdf}
% % \label{fig:cifar_avg_in}
% % }
% % \subfigure[FPR]
% % {\includegraphics[width=0.22\textwidth]{imgs/cifar_avg_out.pdf}
% % \label{fig:cifar_avg_out}
% % }
% \end{minipage}
% \caption{\textbf{Ablation of the effect of using normalization in the features vs. without normalization} considering different OOD datasets on small OOD detection benchmark.}\label{fig:cifar_norm}
% \vspace{-0.2cm}
% \end{figure}

\textbf{Do we need to normalize feature before $k$-nearest neighbors search?} Note that in Algorithm~\ref{alg:main}, before searching the nearest neighbors, we need to normalize the feature vectors by $h_\theta(x) /\parallel h_\theta(x) \parallel_2$. \figurename~\ref{fig:cifar_norm} shows that the normalization process is not necessary for small-scale datasets, and the false positive rate of \abbr without normalization is slightly better than that with normalization. However, without feature normalization, the ID reevaluation accuracy will be greatly reduced. Therefore, in this section, we use feature normalization for experiments as default. The normalization process is more important for large-scale benchmarks, which will be discussed in the next subsection.



\textbf{How to combine the score from $k$ nearest neighbors?} Given a test sample $x_o$ and its $k$-nearest neighbors, we can calculate $k$ score by decreasing order $\left(-\parallel z_o-z_{(1)} \parallel*s_{(1)},...,-\parallel z_o-z_{(k)} \parallel*s_{(k)}\right)$. Here, we compare three different scoring calculation methods: the $k$-th nearest neighbor score ($-\parallel z_o-z_{(k)} \parallel*s_{(k)}$), the average of $k$ nearest neighbor scores ($\frac{1}{k}\sum_{i=1}^k-\parallel z_o-z_{(i)} \parallel*s_{(i)}$), and the median of $k$ nearest neighbor scores ($-\parallel z_o-z_{\lfloor k/2\rfloor} \parallel*s_{\lfloor k/2\rfloor}$), where $\lfloor k/2\rfloor$ is the value of rounding down $k/2$. \figurename~\ref{fig:cifar_avg} shows that $k$ -th score achieves the lowest false positive rate; however, unlike $k$ -avg and $k-$ median scores, the model with $k$-th score cannot identify ID samples successfully, where the precision is usually below $90\%$. $k-$median score achieves high ID accuracy but poor OOD detection results compared to its variants. We choose $k-$avg score as default because it makes a good trade-off between ID reevaluation accuracy and OOD detection performance.

\vspace{-0.15cm}
\subsection{Evaluation and Ablations on Large-scale Out-of-distribution Detection Benchmarks}
\vspace{-0.15cm}
\begin{table}
\centering
\vspace{-0.4cm}
\caption{\textbf{Results on large-scale benchmarks} with ViT-B/16 backbone. The ID dataset is ImageNet and the metric is FPR95.} \label{tab:vit}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
 & \textbf{iNaturalist} & \textbf{SUN} & \textbf{Places} & \textbf{Textures} & \textbf{Avg} \\ \midrule
Mahalanobis & 17.56 & 80.51 & 84.21 & 70.51 & 63.19 \\
KNN & 7.30 & 48.41 & 56.46 & 39.91 & 38.01 \\
\abbr & \textbf{2.37} & \textbf{13.39} & \textbf{24.69} & \textbf{24.01} & \textbf{16.11} \\ \bottomrule
\end{tabular}%
}
\vspace{-0.3cm}
\end{table}
\textbf{Experimental details.} We use a ResNet-50~\cite{he2016deep} backbone by default and train the model by cross-entropy loss. The ImageNet training set~\cite{deng2009imagenet} has $12,800,000$ images with resolution $224\times 224$, making detection tasks more challenging than small-scale experiments. All models are loaded directly from Pytorch~\cite{paszke2019pytorch} and the feature dimension is $2,048$.

\textbf{\abbr reduces the previous best FPR from $53.97$ to $15.97$.} As shown in Table~\ref{tab:imagenet}, utilizing online test samples improve the detection performance by a large margin. Especially on the iNaturalist dataset, FPR is reduced to $1/10$ of the SOTA model. In addition to the surprising performance of OOD detection, \abbr retains a comparable inference time compared to baselines. Besides, \textbf{\abbr benefits from large backbones}. Table~\ref{tab:vit} shows that, with more powerful representations of the ViT-B/16 backbone, the OOD detection performance of \abbr will be further improved. Although some of the baselines can also benefit from better backbones, their performance still have a large gap compared to \abbr.

Due to space limit, we explore various different evaluation protocols in Appendix~\ref{app:sec_settgns}. 

==> sections/intro_icml.tex <==
The classic machine learning models generally suffer from poor performance when the training and test data are not from the same distribution. This vulnerability hinders the deployment of machine learning systems for real-world usage, especially for some safety-critical applications such as autonomous driving~\cite{ramanagopal2018failing}, and biometric authentication~\cite{masi2018deep}. To mitigate the risk of out-of-distribution (OOD) data, the OOD detection problem is studied 
 \cite{hendrycks2016baseline,lee2018simple,yang2021generalized}, which requires an outlier detector to determine whether the input is ID (in-distribution) or OOD. For ID inputs, the system will predict their true class, and  OOD inputs will be reject and not be predicted.

Various methods have been developed to improve the performance of OOD detection, including using the classification confidence or entropy~\cite{hendrycks2016baseline,liu2020energy}, modeling the ID density~\cite{zong2018deep,abati2019latent}, computing the feature distances~\cite{lee2018simple,wang2022vim}, and exposing to OOD samples while training~\cite{hendrycks2018deep}. Despite the encouraging progress, limited performance is achieved for OOD detection for real-world applications, especially for large-scale datasets. For example, for {Large-scale ImageNet Task~\cite{huang2021mos}}, which has $1,280,000$ labeled images, the false positive rate of OOD detection is $53.97\%$ even using the state-of-the-art OOD detection method. The challenge of OOD detection is further highlighted by the impossibility theorem recently developed for OOD detection~\cite{fang2022is}, i.e. it is impossible to reliably detect OOD data points with the access to only ID data points unless further strong assmuption is made. These frustrating results lead to the following fundamental questions:
\begin{center}
\textit{What makes OOD detection so hard, and how to effectively tackle the problem?}
\end{center}



As hinted by the impossiblity theorem from~\cite{fang2022is}, we believe that the fundamental challenge of OOD detection arises from the fact that no OOD data point is available. As a result, a fixed decision criterion is learned from the ID dataset and applied universally regardless of the OOD distribution. To further highlight this limitation, we construct an illustrative example in~\figurename~\ref{fig:motivation} where ID data points are sampled from a normal distribution $\mathcal{N}(0,1)$. Following typical OOD detection methods (e.g.,\cite{sun2022out}), we set the threshold to separate ID/OOD samples as 1.96 since it reaches $95\%$ confidence for the ID distribution.
%If the separation margin is large enough (e.g., situation in~\figurename~\ref{fig:motivation1}), the chosen threshold value produces promising performance. However, 
It works well when the OOD distribution is far from the ID distribution. But when both distributions overlap significantly, as shown in ~\figurename~\ref{fig:motivation2}, this approach will yield a significantly higher false positive rate (near $50\%$) for OOD samples, implying the need to adjust decision criterion based on test samples. One possible solution is to dynamically adjust the threshold based on the test examples that are detected as OOD samples. In particular, for the example illustrated in Figure~\ref{fig:motivation}, using the detected OOD samples, we will be able to decrease the value of the threshold, leading to a significant reduction in false positive rate. 

  
To this end, we follow the fully test-time-adaptation setting~\cite{wang2020tent}. It assumes that test samples come from online data streams and can be used to adjust the model for OOD. Although test-time adaptation (TTA) has been studied before, it is limited to OOD generalization~\cite{zhang2022domain}, domain adaptation~\cite{wang2022continual}, robustness~\cite{wang2020tent}, and long-tailed recognition~\cite{zhang2021test}. To the best of our knowledge, this is the first work that exploits online test samples for OOD detection. 
% \begin{figure}
%  \centering
%  \vspace{-0.1in}  
% \begin{minipage}[t]{\textwidth}        
% \subfigure[$\mathcal{D}^{out}=\mathcal{N}(2,1/2)$]
% {\includegraphics[width=0.22\textwidth]{imgs/motivation2.pdf}
% \label{fig:motivation2}
% }
% \subfigure[$\mathcal{D}^{out}=\mathcal{N}(2,1/2)$]
% {\includegraphics[width=0.22\textwidth]{imgs/motivation_acc2.pdf}
% \label{fig:motivation2_acc}
% }
% \end{minipage}
% \vspace{-0.3cm}
%  \caption{\textbf{The motivation of using test-time adaptation}, where $\mathcal{D}^{in}=\mathcal{N}(0,1)$ and (a) $\mathcal{D}^{out}=\mathcal{N}(2,1/2)$. (b) shows the detection accuracy of both ID and OOD samples, considering different decision boundaries. The decision boundary $x=1.96$ that is learned from only ID data is depicted by the grey dash line. }\label{fig:motivation}
%  \vspace{-0.3cm}
% \end{figure}
\begin{figure}[h]
    \centering
    \minipage{0.23\textwidth}
  \includegraphics[width=0.22\textwidth]{imgs/motivation2.pdf}
\label{fig:motivation2}
\endminipage\hfill
% \minipage{0.32\textwidth}
%   \includegraphics[width=\linewidth]{figs/2tsne_ddg.pdf}
%   %\caption{DDG}
%   \label{fig:tsne_ddg}
% \endminipage\hfill
\minipage{0.23\textwidth}%
  \includegraphics[width=0.22\textwidth]{imgs/motivation_acc2.pdf}
\label{fig:motivation2_acc}
\endminipage
\caption{\textbf{The motivation of using test-time adaptation}, (a) $\mathcal{D}^{in}=\mathcal{N}(0,1)$ and  $\mathcal{D}^{out}=\mathcal{N}(2,1/2)$. (b) shows the detection accuracy of both ID and OOD samples, considering different decision boundaries. The decision boundary $x=1.96$ that is learned from only ID data is depicted by the grey dash line. }
   \label{fig:motivation}
\end{figure}
Intuitively, by leveraging test samples that are labeled as OOD, we can roughly estimate the OOD distribution, and adjust the decision criterion to improve the accuracy of OOD detection. We propose a simple yet effective method, Non-Parametric Test Time Adaptation framework for Out-Of-
Distribution Detection, or \abbr for short, to best leverage online test samples that are pseudo-labeled by the existing decision criterion. Specifically, we construct a feature memory bank to include all feature vectors from training. For a test sample, we compute its score based on its $k$-nearest neighbors from the memory and label it as OOD when the score exceeds a given threshold. Any test sample labeled as OOD is included in the memory bank for future score calculation. To sum up, we make three contributions:


1. We investigate a model-free paradigm to perform TTA by storing features of test instances. The proposed \abbr can be incorporated with any back-end model.

2. We justify the design of \abbr from the viewpoint of a maximum likelihood estimator. Our analysis shows that incorporating online detected OOD instances into decision-making can substantially reduce the false positive rate, especially when In/Out-of-distribution has large overlapping.

3. We conducted experiments on multiple OOD detection benchmarks with $3$ different backbones. Our results show that \abbr can drastically reduce the false positive rate compared to advanced baselines, for example, \abbr reduces the FPR $38\%$ on ImageNet-1k benchmarks. 
% 4. We conduct thorough ablation studies on each component of \abbr. The results shed light on how we choose hyper-parameters considering different scale of datasets.


